Implicit Copulas: An Overview

Implicit copulas are the most common copula choice for modeling dependence in high dimensions. This broad class of copulas is introduced and surveyed, including elliptical copulas, skew $t$ copulas, factor copulas, time series copulas and regression copulas. The common auxiliary representation of implicit copulas is outlined, and how this makes them both scalable and tractable for statistical modeling. Issues such as parameter identification, extended likelihoods for discrete or mixed data, parsimony in high dimensions, and simulation from the copula model are considered. Bayesian approaches to estimate the copula parameters, and predict from an implicit copula model, are outlined. Particular attention is given to implicit copula processes constructed from time series and regression models, which is at the forefront of current research. Two econometric applications -- one from macroeconomic time series and the other from financial asset pricing -- illustrate the advantages of implicit copula models.

==> alm.tex <==
% two new environments for LaTeX
%
% aufgabe - for exercises
% loesung - for solutions
%
% usage:   put a \input{envi.tex} statement in the header of your
%          LaTeX-document, and then simply:
%
%          \begin{aufgabe} text... \end{aufgabe}
%    or    \begin{loesung} text... \end{loesung}

\usepackage{color}
\usepackage{colordvi}
\fboxsep.3cm
\newlength{\breite}
\breite\textwidth
\addtolength{\breite}{-21.78842pt}



\newcounter{aufg}[section]
\newenvironment{aufgabe}%
  {\refstepcounter{aufg}\noindent\textbf{Exercise \arabic{aufg}:}
   \\*[1ex]\noindent}{\vspace{.5cm}}
   
 \newcounter{notes}[section]
\newenvironment{notes}%
  {\refstepcounter{aufg}\noindent\textbf{}
   \\*[1ex]\noindent}{\vspace{.5cm}}
   
   %%%%% Theoreme
\usepackage{amsthm}  % Theoreme
%\usepackage[ngerman]{myproof}  % proof-Umgebung (von Stefan Krause)
%\theorembodyfont{\slshape}  % Nur schr"aggestellt statt kursiv
%\theorembodyfont{\upshape}  % Aufrecht statt kursiv
%\theoremstyle{change}  % Nummer vor die Beschreibung setzen
%\newtheorem{defin}{Definition}[chapter]  % F"ur Numerierung nach \chapter
\newtheorem{defin}{Definition} %[section]  % F"ur Numerierung nach \section
\newtheorem{satz}[defin]{Satz}
%\newtheorem{dsatz}[defin]{Definition und Satz}
\newtheorem{hsatz}[defin]{Hauptsatz}
\newtheorem{theo}{Theorem}
\newtheorem{cor}{Corollary}

\newtheorem{bemer}[defin]{Bemerkung}
%\newtheorem{behau}[defin]{Behauptung}
\newtheorem{lemma}[defin]{Lemma}
\newtheorem{bem}[defin]{Bemerkung}
%\newtheorem{folg}[defin]{Folgerung}
\newtheorem{prop}{Proposition}
%% Dokumentation des Pakets: http://www.tug.org/teTeX/tetex-texmfdist/doc/latex/ntheorem/ntheorem.pdf  


\theoremstyle{definition}
\newtheorem{remark}[]{Remark}
\newtheorem{beisp}[defin]{Example}
\newtheorem*{beisp*}{Example}
\newtheorem{Proof}{Proof}
\makeatletter
\renewenvironment{Proof}[1][\proofname]{\par
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item[\hskip\labelsep
        \itshape
    #1\@addpunct{.}]\mbox{}\par\noindent\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
}
\makeatother



\newtheoremstyle{break}% name
  {}%         Space above, empty = `usual value'
  {}%         Space below
  {}% Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries}% Thm head font
  {.}%        Punctuation after thm head
  {\newline}% Space after thm head: \newline = linebreak
  {}%         Thm head spec
  
\theoremstyle{break}
\newtheorem{Rem}{Remark}

%\newcounter{aufg}[section]
%\newenvironment{aufgabe}%
%  {\refstepcounter{aufg}\noindent\textbf{Aufgabe \arabic{aufg}:}
%   \\*[1ex]\noindent}{\vspace{.5cm}}

%\newcommand{\kopf}[2]%
%{\hrule
%\vspace{.15cm}
%\begin{minipage}{\textwidth}
%{\sfbold Advanced Statistical Inference, Sommersemester 2012, Georg-August-Universit\"at G\"ottingen \hfill
%Blatt #1\\
%Thomas Kneib, Nadja Klein\hfill #2
%}%
%\end{minipage}
%\vspace{.05cm}
%\hrule}

\newcommand{\head}[2]%
 {\hrule \vspace{.15cm} {\sfbold Advanced Statistical Inference, Summer Term 2012, Georg-August-University G\"ottingen}\hfill
{\sfbold Sheet #1}\\
{\sfbold Prof. Dr. Thomas Kneib, Nadja Klein}\hfill {\sfbold #2}

\vspace{.2cm}
\hrule

\vspace{1cm}

}


%%%%%%%%%%%%%%%%%%%%%%%%
% Aufgabenumgebung NEU %
%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{auf}
\newenvironment{auf}%
{\refstepcounter{auf}
\begin{center}
\fcolorbox[gray]{0}{.95}{
\makebox[\breite]{
%\framebox[\textwidth]{
\textbf{Exercise \arabic{auf}}
%}\\*[1ex]\noindent
}}\\*[1ex]\noindent
\end{center}
}{\vspace{.5cm}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Nur ein kleiner Test... %
%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcounter{loes}[section]
\newenvironment{loesung}%
{\stepcounter{loes}
\begin{center}
\fcolorbox[gray]{0}{.95}{
\makebox[\breite]{
\textbf{L"osung \arabic{loes}}
}}\\*[1ex]\noindent
\end{center}
}{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Noch ein kleiner Test... %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newenvironment{material}[1]%
{\begin{center}
\fcolorbox[gray]{0}{.95}{
\makebox[\breite]{
\textbf{Zu Aufgabe #1}
}}\\*[1ex]\noindent
\end{center}\vspace{1cm}
}{\vspace{1cm}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Und noch ein kleiner Test... %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Aufgabenumgebung f\"{u}r Klausuren, nummeriert die Aufgaben und \"{u}bernimmt Punktezahlen...

\newcounter{ka}
\newenvironment{ka}[1]% %Parameter = Punktezahl der Aufgabe
{\refstepcounter{ka}
\begin{center}
\framebox[\textwidth]{
\textbf{Aufgabe \arabic{ka}} \hfill #1 Punkte
}\\*[1ex]\noindent
\end{center}
%\vspace{\fboxsep}
}{\vspace{1cm}}


\newcounter{lka}
\newenvironment{lka}[1]% %Parameter = Punktezahl der Aufgabe
{\refstepcounter{lka}
\begin{center}
\framebox[\textwidth]{
\textbf{L\"osung \arabic{lka}} \hfill #1 Punkte
}\\*[1ex]\noindent
\end{center}
%\vspace{\fboxsep}
}{\vspace{1cm}}

% that's it.


==> append_esn.tex <==
%\newpage
%\appendix

\noindent

\section{}\label{app:postN}
This appendix provides the MCMC sampler for drawing from
the posterior of $\varthetavec=\lbrace\betavec,\sigma^2,\tau^2\rbrace$ in the Gaussian probabilistic 
ESN for a given configuration $\xivec$, and the algorithm for simulating draws from forecast distribution.

\noindent \underline{Algorithm~1} {\em (MCMC sampler for Gaussian probabilistic ESN)}\\
\noindent
Repeat the following steps sequentially:
\begin{itemize}
\setlength{\itemindent}{0.5cm}
\item[1.] Generate from $\betavec|\{\varthetavec\setminus\betavec\},X,\yvec$.
\item[2.] Generate from $\sigma^2|\{\varthetavec\setminus\sigma^2\},X,\yvec$.
\item[3.] Generate from $\tau^2|\{\varthetavec\setminus\tau^2\},X,\yvec$.%Perform MH-step for $\tau^2$
\end{itemize}

\noindent 
The conditional posteriors above are standard and their derivation is omitted here.
% At Step~1
%$\betavec\sim\mathcal{N}_p(\muvec_{\beta},\Sigma_{\beta})$, with
% $\Sigma_{\beta}=(B_\xi(X)'B_\xi(X)/\sigma^2+1/\tau^2 I)^{-1}$ and $\mu_{\beta}=\Sigma_{\beta}B_\xi(X)'\yvec/\sigma^2$. At Steps~2 and~3
% the distributions are inverse Gammas, where
%$\sigma^2\sim\mathcal{IG}(a+\frac{T}{2},b+\frac{1}{2}\varepsilonvec'\varepsilonvec)$
%and 
%$\tau^2 \sim\mathcal{IG}(\tilde a+\frac{p}{2},\tilde b+\frac{1}{2}\betavec'\betavec)$,
%with $p=\dim(\betavec)$. 
The scheme is very fast and
converges quickly. Accurate mixture estimates of the 
posterior mean $\hat{\varthetavec}=E(\varthetavec|X,\yvec)$ 
can be computed from a few hundred draws post-convergence.

Algorithm~2 below is used to simulate from the ensemble forecast distribution
at~(5). Let 
$y^r_{i,t}$ denote the $i$th Monte Carlo draw of (logarithmic) price
in region $r\in\{1,2,\ldots,5\}$ at time $t$. For time points $t\leq T$,
this is simply set equal to its in-sample observed value,
but for each point $t> T$, $i=1,\ldots,N$ different values are drawn. 
In Algorithm~2 we use
subscript $i$ and superscript $r$ to indicate quantities that correspond to draw $i$ 
for region $r$.  


\noindent \underline{Algorithm~2} {\em (Generating from the Gaussian ESN ensemble predictive distributions)}\\
\noindent
For each ESN configuration $\xivec^{1},\ldots,\xivec^{K}$ repeat the following:
\begin{itemize}
	\setlength{\itemindent}{0cm}
	\item[1.] For each of the five regional price series, compute $\hat{\varthetavec}^r$ using Algorithm~1.
	\item[2.] For $i=1,\ldots,N$, $t=T+1,\ldots,T+h_1$, and $r=1,\ldots,5$ do:
	\begin{itemize}
		\item[2.1] Construct $\xvec^r_{i,t}$ from previous series values $\{y^d_{i,s}\,;d=1,\dots,5,\,s=1,\ldots,t-1\}$
		\item[2.2] Compute $\hvec^r_{i,t}$ from $\{\hvec^r_{i,t-1},\xvec^r_{i,t}\}$ using the hidden state equation at~(1) in the main paper.
%		\item[2.3] Set $\bvec_{i,t}^r=\left[(\hvec_{i,t}^r)',((\hvec^r_{i,t})^{\circ 2})'\right]$
		\item[2.3] Draw $y_{i,t}^r$ from $\mathcal{N}(\hvec_{i,t}^r\hat{\betavec}_1^r+(\hvec_{i,t}^r)^{\circ 2}\hat{\betavec}_2^r,(\hat{\sigma}^2)^r)$ and store
		in an $(K N\times h_1 \times 5)$ array
	\end{itemize}
\end{itemize}

Algorithm~2 can be run in parallel 
over the $K$ configurations, while step~2.1 is undertaken using 
the
feature vector specification in Sec.~5.1 of the main paper. The algorithm produces
$KN$ draws from the joint ensemble forecast distribution of 
$(\bm{Y}_{\mbox{\tiny ALL},T+1},\ldots,\bm{Y}_{\mbox{\tiny ALL},T+h_1})$ of the 
Gaussian probabilistic 
ESN model. The $KN$ draws of each element in this vector
are from a marginal forecast distribution with ensemble density at~(5) of the main paper. 
In our empirical work we set $K=100$, $N=20$ and $h_1=24$, providing a total of $KN=2000$ draws for a vector of $5h_1=120$ future values. 
We run Algorithm~2 for each forecast origin in our evaluation period.
%Simply computing $\mbox{Price}^r_{i,t}=\exp(y^r_{i,t})-1001$
%converts these to draws from the forecast distribution of the
%nominal dollar-valued price processes.

\section{}\label{app:postST}
This appendix provides the MCMC sampler for drawing from
the posterior of $\varthetavec=\lbrace\betavec,\tau^2,\psi,\sigma^2\rbrace$ in the skew $t$ probabilistic 
ESN, augmented with 
the latent variables $\zetavec,\wvec$, for a given configuration $\xivec$.
The initial values for the parameters are $\sigma^2=c_0/(C_0+1)$ (prior mode), $\betavec=\nullvec$,  $\tau^2=0.1$,  $\psi=0$, $\zetavec=\nullvec$, $\wvec=\onevec$.

\noindent \underline{Algorithm~3} {\em (MCMC sampler for skew $t$ probabilistic ESN)}\\
\noindent
Repeat the following steps sequentially:
\begin{itemize}
	\setlength{\itemindent}{0.5cm}
	\item[1.] Generate from $\betavec|\{\varthetavec\setminus\betavec\},\wvec,\zetavec,X,\yvec$
	\item[2.] Generate from $p(\psi|\{\varthetavec\setminus\psi\},\wvec,\zetavec,X,\yvec)$
	\item[3.] Generate from $p(\sigma^2|\{\varthetavec\setminus\sigma^2\},\wvec,\zetavec,X,\yvec)$
	\item[4.] Generate from $p(\tau^2|\{\varthetavec\setminus\tau^2\},\wvec,\zetavec,X,\yvec)$
	\item[5.] For $t=1,\ldots,T$ generate from $p(\zeta_t|\varthetavec,w_{t},X_t,y_{t})$
	\item[6.] For $t=1,\ldots,T$ generate from $p(w_{t}|\varthetavec,\zeta_t,X,y_{t})$
\end{itemize}

\noindent 
All the conditional densities in steps~1 to 6 can be computed readily in 
closed form. In step~1, $\betavec\sim\mathcal{N}_p(\muvec_{\beta},\Sigma_{\beta})$
where $\Sigma_{\beta}=(B_\xi(X)'W B_\xi(X)/\sigma^2+1/\tau^2 I)^{-1}$, $\muvec_{\beta}=\Sigma_{\beta}(B_\xi(X)'W(\yvec-\psi\zetavec))/\sigma^2$
and $W=\mbox{diag}(\wvec)$ is a diagonal matrix of the latent variables.
At step~2,	$\psi\sim\mathcal{N}_1(\mu_{\psi},\sigma^2\sigma_{\psi})$,
where
$\sigma_{\psi}=(\zvec'W \zvec/\sigma^2+1/D_0)^{-1}$ and $\mu_{\psi}=\sigma_{\psi}(\zvec'W(\yvec-B_\xi(X)\betavec))/\sigma^2$. 
At step~3, 
$\sigma^2\sim\mathcal{IG}(c_k,C_k)$ with $C_k=C_0+\frac{1}{2}\left(\epsilonvec'W\epsilonvec+\frac{\psi^2}{D_0}\right)$, $\epsilon_{t}=y_{t}-b_{t}'\betavec-\psi \zeta_t$, $\epsilonvec=(\epsilon_{1},\ldots,\epsilon_{T})'$ and $c_k=c_0+\frac{1}{2}(T+1)$. At step~4, $\tau^2\sim\mathcal{IG}(b_k,B_k)$,
with $B_k=B_0+\frac{1}{2}\betavec'\betavec$ and $n_k=(b_0+p/2)$.
At step~5, $\zeta_t\sim\mathcal{TN}_{[0,\infty)}(a_{t},A/w_{t})$ with
$A=(1+\psi^2/\sigma^2)^{-1}$ and
$a_{t}=A\psi(y_{t}-B_\xi(X)'\betavec)/\sigma^2$. Finally, at step~6,
$w_{t}\sim\mathcal{G}(\nu/2+1,(\nu+\zeta_t^2+\epsilon_{t}^2/\sigma^2)/2)$,
where $\mathcal{G}$ denotes a gamma distribution.

%\begin{itemize}
%	\item[Step 1.] 
%	\[
%	\betavec|\lbrace\varthetavec\setminus\betavec\rbrace,\wvec,\zetavec,X,\yvec\sim\mathcal{N}_p(\muvec_{\beta},\Sigma_{\beta}),
%	\]
%	where $\Sigma_{\beta}=(B_\xi(X)'W B_\xi(X)/\sigma^2+1/\tau^2 I)^{-1}$, $\mu_{\beta}=\Sigma_{\beta}(B_\xi'W(\yvec-\psi\zetavec))/\sigma^2$
%	and $W=\mbox{diag}(w_1,\ldots,w_T)$ is a diagonal matrix of the latent variables.
%	\item[Step 2.]
%	\[
%	\psi|\lbrace\varthetavec\setminus\psi\rbrace,\wvec,\zetavec,X,\yvec\sim\mathcal{N}_p(\muvec_{\psi},\sigma^2\Sigma_{\psi}),
%	\]
%	where $\Sigma_{\psi}=(z'W z/\sigma^2+1/D_0)^{-1}$ and $\mu_{\psi}=\Sigma_{\psi}(z'W(\yvec-B_\xi(X)\betavec))/\sigma^2$. 
%	\item[Step 3.] 
%	\[
%	\sigma^2|\lbrace\varthetavec\setminus\sigma^2\rbrace,\wvec,\zetavec,X,\yvec\sim\mathcal{IG}(c_k,C_k),
%	\]
%	where $C_k=C_0+\frac{1}{2}\left(\epsilonvec'W\epsilonvec+\frac{\psi^2}{D_0}\right)$, $\epsilon_{t}=y_{t}-b_{t}'\betavec-\psi \zeta_t$, $\epsilonvec=(\epsilon_{1},\ldots,\epsilon_{T})'$ and $c_k=c_0+\frac{1}{2}(T+1)$.
%	\item[Step 4.] 
%	\[
%	\tau^2|\lbrace\varthetavec\setminus\tau^2\rbrace,\wvec,\zetavec,X,\yvec\sim\mathcal{IG}(b_k,B_k),
%	\]
%	where $B_k=B_0+\frac{1}{2}\betavec'\betavec$,  and $n_k=(b_0+p/2)$, as well as $p=\dim(\betavec)$.
%	%To perform a MH-step for the current value for $\tau^2$ we use the same Gaussian IWLS proposal for $log(\tau^2)$ as for the RNN and RNNC.
%	\item[Step 5.]  
%	\[
%	\zeta_t|\varthetavec,w_{t},\xvec_t,\yvec_{t}\sim\mathcal{TN}_{[0,\infty)}(a_{t},A/w_{t}),
%	\]
%	where 
%	\[
%	A=(1+\psi^2/\sigma^2)^{-1},\quad a_{t}=A\psi(y_{t}-B_\xi(X)'\betavec)/\sigma^2.
%	\]
%	\item[Step 6.] 
%	\[
%	w_{t}|\varthetavec,\zeta_t,\xvec_t,\yvec_{t}\sim\mathcal{G}\left(\frac{\nu}{2}+1,\frac{\nu+\zeta_t^2+\epsilon_{t}^2/\sigma^2}{2}\right).
%	\]
%%\end{itemize}
%After convergence, Algorithm~3 produces a Monte Carlo sample from the 
%augmented posterior distribution $\varthetavec,\wvec,\zetavec|X,\yvec$.

To simulate Monte Carlo draws from the ensemble forecast distribution at~(5) in the main paper,
Algorithm~2  is employed with minor adjustments. First, at step~1
the estimate $\hat{\varthetavec}^r$ is computed using Algorithm~3 above. 
Second, at step~2.3 
the iterate $y_{i,t}^r$ is drawn from a
$\mathcal{ST}(\hvec_{i,t}^r\hat{\betavec}_1+(\hvec_{i,t}^{r})^{\circ 2}
\hat{\betavec}_2^r,(\hat \omega^2)^r,\hat \alpha^r,\hat \nu^r)$ 
distribution. Here, at each sweep of Algorithm~3 draws of $\omega,\alpha$ are obtained from that of $\varthetavec$ as 
$\alpha=\psi/\sigma$ and $\omega=(\sigma^2+\psi^2)^{1/2}$, and 
the means of these draws computed to obtain $\hat \omega^r,\hat \alpha^r$. 

\section{}\label{app:postcop}
This appendix outlines the MCMC sampler for drawing from the 
posterior of $\varthetavec=\lbrace\betavec,\tau^2\rbrace$ in the deep copula model
for a given configuration $\xivec$. An algorithm for drawing from ensemble forecast distribution from the copula model is also given.

\noindent \underline{Algorithm~4} {\em (MCMC sampler for the deep copula)}\\
\noindent
Repeat the following steps sequentially:
\begin{itemize}
	\setlength{\itemindent}{0.5cm}
	\item[1.] Generate from $\betavec|\tau^2,X,\yvec$
	\item[2.] Generate from $\log(\tau^2)|\betavec,X,\yvec$
\end{itemize}
%\item[\textbf{Starting values}] For starting values we set $\betavec^{(0)}=\nullvec$,  $(\tau^2)^{(0)}=1$.

\noindent At step~1,
$\betavec\sim\mathcal{N}_p(\muvec_{\beta},\Sigma_{\beta})$, with
$\Sigma_{\beta}=(B_\xi(X)'B_\xi(X)+1/\tau^2 I)^{-1}$ and $\mu_{\beta}=\Sigma_{\beta}B_\xi(X)'\zvec$.  A Metropolis-Hastings step 
is used to generate $\upsilon=\log(\tau^2)$ at step~2, with
a Gaussian proposal with matching mode and curvature. Note that from
the conditional likelihood in Sec.~4.4, 
\begin{equation*}\label{eq:logFC:upsilon}
  \begin{aligned}
	  &l_{\upsilon}\equiv \log(p(\upsilon|X,\betavec,\yvec))\propto -\frac{\upsilon}{2}\left(\dim(\betavec)))-1\right)-\frac{1}{2\exp(\upsilon)}\betavec'\betavec-\left(\frac{\exp(\upsilon)}{b_{\tau^2}}\right)^{\tfrac{1}{2}}\\&
\quad\quad\quad\qquad\qquad\qquad\quad\;\,-\frac{1}{2}\sum_{i=1}^{n}\log(s_i^2)
-\frac{1}{2}\left(\zvec'(SS')^{-1}\zvec-2\betavec'B_\xi(X)'S^{-1}\zvec\right)\,.
  \end{aligned}
\end{equation*}
Approximating $l_{\upsilon}$ by a second order Taylor expansion around the current state $\upsilon^{(c)}$,
and taking the exponent, yields the proposal density $\ND\left(\mu_{\upsilon},\sigma_{\upsilon}^2\right)$ with
%\begin{equation*}\label{eq:param:proposal:tau2}
 $\mu_{\upsilon}=\sigma_{\upsilon}^2\frac{\partial l_{\upsilon}}{\partial\upsilon}+\upsilon$ and $\sigma_{\upsilon}^2=-1/\frac{\partial^2 l_{\upsilon}}{\partial\upsilon^2}.$
The derivatives in the proposal density for can be computed quickly in closed form
as
\begin{equation*}%\label{app:eq:deriv:tau2}
  \begin{aligned}
    \frac{\partial l_{\upsilon}}{\partial\upsilon}&= -\frac{1}{2}\left(\dim(\betavec)-1\right)+\frac{1}{2\exp(\upsilon)}\betavec'\betavec-\left(\frac{\exp(\upsilon)}{4b_{\tau^2}}\right)^{\tfrac{1}{2}}\\&\quad-\frac{1}{2}\sum_{i=1}^{n}\frac{1}{s_i^2}\frac{\partial}{\partial\upsilon}s_i^2 -\frac{1}{2}\left(\zvec'\left\lbrack\frac{\partial}{\partial\upsilon}(SS')^{-1}\right\rbrack\zvec-2\betavec'B_\xi(X)'\left\lbrack \frac{\partial}{\partial\upsilon}S^{-1}\right\rbrack\zvec\right)\\
    \frac{\partial^2 l_{\upsilon}}{\partial\upsilon^2}&= - \frac{1}{2\exp(\upsilon)}\betavec'\betavec-\left(\frac{\exp(\upsilon)}{16b_0}\right)^{\tfrac{1}{2}}-\frac{1}{2}\sum_{i=1}^{n}\left(\left\lbrack \frac{\partial}{\partial\upsilon}\frac{1}{s_i^2}\right\rbrack\frac{\partial}{\partial\upsilon}s_i^2+\frac{1}{s_i^2}\frac{\partial^2}{\partial\upsilon^2}s_i^2\right)\\&\quad -\frac{1}{2}\left(\zvec'\left\lbrack\frac{\partial^2}{\partial\upsilon^2}(SS')^{-1}\right\rbrack\zvec-2\betavec'B_\xi(X)'\left\lbrack \frac{\partial^2}{\partial\upsilon^2} S^{-1}\right\rbrack\zvec\right)\,.
  \end{aligned}
\end{equation*}
where the partial derivatives above are simple closed form expressions.

Algorithm~5 below is used to generate draws from the ensemble forecasting 
distribution at~(5) of the main paper for the deep copula model. It is an adjustment
of Algorithm~2 used for the probabilistic Gaussian ESN, with
similar super- and sub-script notation. Let 
$z_{i,t}^r$ denote the $i$th Monte Carlo draw of the (standardized)
pseudo-response in region $r\in\{1,\ldots,5\}$ at time $t$. For time points $t\leq T$, 
this is set equal to its in-sample value computed once as $z_{i,t}^r=\Phi_1^{-1}(F_Y(y^r_{t}))$. For time points $t>T$, $i=1,\ldots,N$ values
 are drawn for each ESN configuration.

\noindent \underline{Algorithm~5} {\em (Generating from the deep copula model ensemble predictive distributions)}\\
\noindent
For each ESN configuration $\xivec^{1},\ldots,\xivec^{K}$ repeat the following:
\begin{itemize}
	\setlength{\itemindent}{0cm}
	\item[1.] For each of the five regional price series, compute $\hat{\varthetavec}^r$ using Algorithm~4.
	\item[2.] For $t=1,\ldots,T$ and $r=1,\ldots,5$, compute $z_{i,t}^r=\Phi_1^{-1}(F_Y(y_{t}^r))$.
	\item[3.] For $i=1,\ldots,N$, $t=T+1,\ldots,T+h_1$, and $r=1,\ldots,5$ do:
	\begin{itemize}
		\item[3.1] Construct $\xvec^r_{i,t}$ from previous values $\{z^d_{i,s}\,;d=1,\dots,5,\,s=1,\ldots,t-1\}$.
		\item[3.2] Compute $\hvec^r_{i,t}$ from $\{\hvec^r_{i,t-1},\xvec^r_{i,t}\}$ using the hidden state equation at~(1).
		\item[3.3] Set $\bvec_{i,t}^r=\left[(\hvec_{i,t}^r)',((\hvec^r_{i,t})^{\circ 2})'\right]$ and compute $\psi_{i,t}^r=
		(1+\tau^2 \bvec_{i,t}^r(\bvec_{i,t}^r)')^{-1/2}$.
		\item[3.4] Draw $z_{i,t}^r$ from $\mathcal{N}(\psi_{i,t}^r\bvec_{i,t}^r \hat{\betavec}^r,(\psi_{i,t}^r)^2)$.
		\item[3.5] Set $y_{i,t}^r=F_Y^{-1}(\Phi_1(z_{i,t}^r))$ and store
		in an $(KN\times h_1 \times 5)$ array.
	\end{itemize}
\end{itemize}
Algorithm~5 can be run in parallel 
over the $K$ configurations, while step~3.1 is undertaken using 
the
feature vector specification in Sec.~5.1. The algorithm produces
$KN$ draws from the joint ensemble forecast distribution of 
$(\bm{Y}_{\mbox{\tiny ALL},T+1},\ldots,\bm{Y}_{\mbox{\tiny ALL},T+h_1})$ 
for the deep copula model. The $KN$ draws of each element in this $5h_1 \times 1$ vector
are from a marginal distribution with ensemble density of the
form at~(5) in the main paper. We use Algorithm~5 at each forecast origin in our evaluation period.

==> append_isf.tex <==
\appendix
\noindent {\bf \Large{Appendix}}\\
\vspace{-20pt}

\noindent {\bf \large{Part~A}}\\
\noindent 
This part of the appendix outlines how to efficiently evaluate
the quantile function $F_{Z_1}^{-1}$
and
the logarithm
of the marginal
density $\log(f_{Z_1}(z))$ for a stationary nonlinear state space model.
For both, we
use spline interpolations
based on their values at $N$ absciassae, where
we set $N=100$ in practise.
The advantage of such spline-based approximations is that they are
highly accurate (between 5 and 9 decimal places in our empirical
work), 
yet are fast to compute at the $T$ observations once
the interpolation is complete-- even for large values of $T$.

We use a uniform grid for the $N$
quantile
function values
$\{q_1,\ldots,q_N\}$, which have correpsonding probability values
$\{p_1,\ldots,p_N\}$. 
We set $p_1=0.0001$ and $p_N=0.9999$, so that
the function is approximated far into the tails of the distribution.
The following steps obtain the 
points at which the interpolations are made.
\begin{itemize}
\setlength\itemsep{-0.5em}
\item[1.] Set $p_1=0.0001$ and $p_N=0.9999$, and evaluate both
$q_1=F_{Z_1}^{-1}(p_1)$ and $q_N=F_{Z_1}^{-1}(p_N)$
using a root finding algorithm.
\item[2.] Set step size to $\delta=(q_N-q_1)/(N-1)$, and a construct
uniform grid as $q_i=q_1+(i-1)\delta$, for $i=2,\ldots,N$.
\item[3.] For $i=1,\ldots,N$ (in parallel): \\
\indent \indent 3a. Compute $p_i=F_{Z_1}(q_i)$\\
\indent \indent 3b. Compute $b_i=\log(f_{Z_1}(q_i))$
\end{itemize}

We then interpolate the points $\{(p_i,q_i);i=1,\ldots,N\}$
and $\{(q_i,b_i);i=1,\ldots,N\}$ using splines. We employ
natural cubic smoothing splines 
using the (fast and efficient)
spline toolbox in MATLAB, although other fast interpolating methods
could also be employed. 
Notice that
numerical
inversion of $F_{Z_1}$ is undertaken above only twice in Step~1. Moreover,
$F_{Z_1}$ and $f_{Z_1}$ are evaluated
only $N$ times in step~3, something
that can also be undertaken parallel.

If the marginal distribution $F_{Z_1}$ is symmetric,
as in Section~\ref{sec:sv}, then
$F_{Z_1}^{-1}(1-u)=-F_{Z_1}^{-1}(u)$ for $0\leq u\leq 1/2$, 
$f_{Z_1}(z)=f_{Z_1}(-z)$ and
$F_{Z_1}(-z)=1-F_{Z_1}(z)$ for $z\geq 0$. These identities can be exploited
to reduce the number of computations at Steps~1 and~3 by one half, further
speeding the algorithm.
 
To illustrate the effectiveness of the method, we consider the approximations
to $F_{Z_1}^{-1}$ and $\log(f_{Z_1})$ 
when $\bm{\psi}$ equals the
posterior mean in the inflation study
in Section~\ref{sec:inflsv}.
Plots of the approximations are visually
indistinguishable from the true functions,
which can be evaluated (slowly) using numerical methods. The integrated
absolute error between the approximate and true functions are 
$7.9\times 10^{-6}$ and $3.6\times 10^{-6}$ for the quantile and log-density,
respectively.
Computation of
both
approximations, and their evaluation at the $T=240$ observations, 
takes only 0.29s using MATLAB on a standard four core desktop.

\noindent {\bf \large{Part~B}}\\
\noindent 
This part of the appendix shows how to evaluate the bivariate marginal
copula density
\[
c^{(2)}(u_1,u_2;\bm{\psi})=
\frac{f_Z^{(2)}(z_1,z_2|\bm{\psi})}{f_{Z_1}(z_2|\bm{\psi})f_{Z_1}(z_1|\bm{\psi})}\,,
\]
for InvCop1 and InvCop2. In both cases,
the univariate marginal density
$f_1(z|\bm{\psi})$ can be computed readily as in Part~A above.
Computation of $f_Z^{(2)}$ is outlined
separately for each case below. 

\noindent {\bf For InvCop1}\\
\noindent
For the SVUC model with the parameter constraints, the bivariate
density 
\[f^{(2)}_Z(z_1,z_2|\bm{\psi})=\int\int\int\int 
	\phi_2\left(\bm{z};\bm{\mu},V(\bm{\zeta})\right)\,
\phi_2(\bm{\mu};\bm{0},S_\mu)\mbox{d}
\bm{\mu}\,\phi_2(\bm{\zeta};(\bar \zeta ,\bar \zeta),S_\zeta) \mbox{d}\bm{\zeta}\,,
\]
where
$\bm{z}=(z_1,z_2)$, $\bm{\mu}=(\mu_1,\mu_2)$, $\bm{\zeta}=(\zeta_1,\zeta_2)$,
\[
V(\bm{\zeta})=\left[\begin{array}{cc} \exp(\zeta_1)& 0\\ 0& \exp(\zeta_2) \end{array}\right],\,
S_\zeta=s_\zeta^2\left[\begin{array}{cc} 1& \rho_\zeta\\ \rho_\zeta& 1 \end{array}\right],\,
S_\mu=s_\mu^2\left[\begin{array}{cc} 1& \rho_\mu\\ \rho_\mu& 1 \end{array}\right],\, 
\]
and $\phi_2(\bm{x};\bm{a},\Omega)$ is a bivariate normal density
with mean $\bm{a}$ and variance $\Omega$
evaluated at point $\bm{x}$.
The inner two integrals in $\bm{\mu}$ of this 4-dimensional integral
can be computed analytically by recognising a bivariate normal.
Then, by recognising a second bivariate normal in
$\bm{z}$, the density can be written as:
\[f(z_1,z_2|\bm{\psi})=\int\int \phi_2(\bm{z};\bm{0},W(\bm{\zeta}))\phi_2(\bm{\zeta};(\bar \zeta,\bar \zeta),S_\zeta)
\mbox{d}\bm{\zeta}\,,
\]
where $W(\bm{\zeta})=(S_\mu+V(\bm{\zeta}))$. This bivariate integral can be
computed numerically.

\noindent {\bf For InvCop2}\\
\noindent 
For the MSAR1 model with the parameter constraints, the bivariate density 
is the mixture of four bivariate Gaussians
\begin{eqnarray*}
f^{(2)}_Z(z_1,z_2|\bm{\psi})=\sum_{i=1,2}\sum_{j=1,2}\phi_2 
\left( (z_1,z_2);\bm{\mu}_{ij},
S_{ij} \right)p_{ij}\pi_i\,,
\end{eqnarray*}
where $\bm{\mu}_{ij}=\left(\mu_i,\mu_j\right)$ and
\[
S_{ij}=\begin{bmatrix} s^2_i & \rho_j s^2_i \\ \rho_j s^2_i & s^2_j \end{bmatrix}\,.
\] 


==> figs.tex <==






